Probabilistic Permutation Graph Search: Black-Box Optimization for Fairness in Ranking

There are several measures for fairness in ranking, based on different underlying assumptions and perspectives. PL optimization with the REINFORCE algorithm can be used for optimizing black-box objective functions over permutations. In particular, it can be used for optimizing fairness measures. However, though effective for queries with a moderate number of repeating sessions, PL optimization has room for improvement for queries with a small number of repeating sessions. In this paper, we present a novel way of representing permutation distributions, based on the notion of permutation graphs. Similar to PL, our distribution representation, called PPG, can be used for black-box optimization of fairness. Different from PL, where pointwise logits are used as the distribution parameters, in PPG pairwise inversion probabilities together with a reference permutation construct the distribution. As such, the reference permutation can be set to the best sampled permutation regarding the objective function, making PPG suitable for both deterministic and stochastic rankings. Our experiments show that PPG, while comparable to PL for larger session repetitions (i.e., stochastic ranking), improves over PL for optimizing fairness metrics for queries with one session (i.e., deterministic ranking). Additionally, when accurate utility estimations are available, e.g., in tabular models, the performance of PPG in fairness optimization is significantly boosted compared to lower quality utility estimations from a learning to rank model, leading to a large performance gap with PL. Finally, the pairwise probabilities make it possible to impose pairwise constraints such as "item $d_1$ should always be ranked higher than item $d_2$." Such constraints can be used to simultaneously optimize the fairness metric and control another objective such as ranking performance.

==> sections/unused.tex <==
Before formally defining~\ac{PPG}, we need to define \emph{support edges} of an edge in the permutation graph.
We write $\mathscr{P}_D$ for the collection of all possible permutation graphs over a list of items $D=[d_1, d_2, \dots, d_n]$.

\begin{definition}{\bfseries Support edges.}
\label{def:supportset}
    For an edge $e_{ij}=(d_i, d_j)$, we write $P_{ij}$ for the set of permutation graphs containing $e_{ij}$:
    \begin{equation*}
        P_{ij}=\left\{G \in \mathscr{P}_D : e_{ij} \in E_G\right\},
    \end{equation*}
    \noindent
    and $\bar{P}_{ij}$ for the set of minimal graphs of $P_{ij}$: no proper subgraph of graphs in $\bar{P}_{ij}$ are in $P_{ij}$
    The set of support edges of $e_{ij}$ is constructed as follows:
    \begin{equation*}
        S_{ij} = \left\{ E\left(G\right)-e_{ij} : G \in \bar{P}_{ij}\right\}.
    \end{equation*}

\end{definition}

Remember that each edge in a permutation graph represents an inversion between its two endpoints.
If the set of support edges of an edge is not empty, it means that the inversion of its two endpoints depends on other inversions, without which the resulting graph would not be a valid permutation graph.
Let's clarify this by a toy example.

\begin{example}
    \label{exa:supportedges}
Assume that $D=[d_1, d_2, d_3, d_4]$.
It is easy to see that 
\begin{equation*}
    S_{12}=S_{23}=S_{34} = \emptyset,
\end{equation*}
as inverting two consecutive items can be done without the need to invert other items.
However, inverting $d_1$ and $d_3$ cannot be done without affecting $d_2$.
\input{sections/figure_tex/03-fig-supportedges}
Simple calculations show that
\begin{equation*}
    S_{13}=\big\{\left\{e_{12}\right\}, \left\{e_{23}\right\}\big\}\quad;\quad
    S_{24}=\big\{\left\{e_{23}\right\}, \left\{e_{34}\right\}\big\}.
\end{equation*}
In other words, inverting $d_1$ and $d_3$ requires either an inversion between $d_1$ and $d_2$ or $d_2$ and $d_3$.
Finally, we have
\begin{equation*}
    S_{14}=\big\{
        \left\{e_{12}, e_{13}\right\}, 
        \left\{e_{12}, e_{34}\right\}, 
        \left\{e_{34}, e_{24}\right\},
        \left\{e_{23}, e_{13}, e_{24}\right\}\big\}.
\end{equation*}
Fig.~\ref{fig:supportedges} shows three cases from the above example.
In each graph, the dotted edges are the support edges for the solid edge.

\end{example}








\begin{definition}{\bfseries \Acf{PPG}.}
    \label{def:ppg}
        Given a list of items $D$ and a reference permutation $\pi_0$ on $D$, a corresponding~\ac{PPG} is a weighted complete graph $G=(D,E,w)$, whose edges are weighted by a probability value obtained from $w:E\rightarrow[0,1]$.
        Sequentially, each edge goes through a Bernoulli sampling and is selected with a success probability given by its weight.
        The sampling order of edges is such that an edge goes through the sampling only if at least one set of its support edges has already been completely selected.
        As such, $w(e)$ indicates the conditional probability of sampling $e$, conditioned on having at least one set of the support edges of $e$ already completely sampled.
    \end{definition}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Efficient Sampling of Permutation Graph}
\label{sec:method:samplingpermutationgraph}
We denote by \emph{realization} the process of sampling the edges from the~\ac{PPG} to realize a permutation graph.
Each edge should go through the sampling only if at least one of its support sets is completely covered in the realization so far; otherwise, its inclusion in the realized graph makes it non-permutation (see Definition~\ref{def:supportset}).
As such, there should be an ordering for the edges to sample: the edges in the support sets of edge $e$ should be placed before $e$ in the ordering.

The idea is to start sampling from the edges with empty support sets and add new eligible candidates to the sampling queue each time a new edge is sampled.
Before formally presenting the method, let us first elaborate it by an example.

\begin{example}
    \label{exa:samplingpermutationgraph}
Assume that $D=[d_1, d_2, d_3, d_4]$.
Edges with two consecutive items as endpoints, namely $e_{12}$, $e_{23}$ and $e_{34}$, have empty support sets and can be considered for sampling.
We use a Bernoulli random variable to sample each edge with its corresponding probability.
Assume that only the $e_{23}$ edge is selected for inclusion in the realized permutation graph.
Inverting $d_2$ and $d_3$ allows both $e_{13}$ and $e_{24}$ to be eligible for sampling: $\{e_{23}\}$ covers one of the sets in both $S_{13}$ and $S_{24}$.
Finally, the $e_{14}$ edge would be eligible for sampling only if both $e_{13}$ and $e_{24}$ are included in the realized graph, as this is the only way that one of the sets in $S_{14}$ is covered.
This process can be summarized by the following diagram:
\begin{equation*}
    [1,2,3,4] \rightarrow 
    [1,\underline{3,2},4] \rightarrow 
    [\underline{3,1},\underline{4,2}] \rightarrow 
    [3,\underline{4,1},2]
\end{equation*}

\end{example}

Our method for sampling has similarities with bubble sort \todo{[ref]}, as can be seen from the above example.
We start by adding consecutive items to the list of eligible inversions.
At each step, we pick an edge from the eligible list and use a Bernoulli random variable to decide if it should be added to the realized permutation graph or not.
Each time an edge $(d_{i_1}, d_{i_2})$ is added to the partially realized graph, the permutation is updated by inverting its two endpoints:
\begin{equation*}
    [\cdots, d_{i_0}, d_{i_1}, d_{i_2}, d_{i_3}, \cdots] \rightarrow
    [\cdots, d_{i_0}, \underline{d_{i_2}, d_{i_1}}, d_{i_3}, \cdots]
\end{equation*}
and two new eligible edges are added to the list: $(d_{i_0}, d_{i_2})$ and $(d_{i_1}, d_{i_3})$.
One important thing to note here is that after swapping $d_{i_1}$ and $d_{i_2}$, previously eligible $(d_{i_0}, d_{i_1})$ and $(d_{i_2}, d_{i_3})$ are no longer eligible.
The realization process is continued as above, until the eligible list becomes empty.

\input{sections/figure_tex/03-alg-sampling}

The pseudo-code for this method is depicted in Alg.~\ref{alg:sampling}.
In this pseudo-code, $L$ is the eligible list of the edges.
We only store the first endpoints in $L$, since the inversions only happen between consecutive items in the updated permutation (Line $9$).
In Line $11$, after a successful inversion, we exclude $i-1$ and $i+1$ from the eligible list, because
inverting items $i$ and $i+1$ \todo{diminishes} the possibility of inverting either $i-1$ and $i$ or $i+1$ and $i+2$: They are no longer consecutive items.
For the same reason, in line $5$, we randomly pick from the eligible list: If we pick sequentially from $L$, the items at the front of the $L$ will have a higher chance to be inverted than the rear items.

Next, we will present the main part of our~\ourmethod method which is learning the weights of the~\ac{PPG}, based on the objective function.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Learn Graph Weights}
\label{sec:method:learngraph}

Each~\ac{PPG} defines a distribution over permutation graphs.
We are interested in finding a distribution where the highly probable permutations lead to near optimum values for the objective function.
As we use~\ac{PPG} to search in the permutation space, we call our method~\emph{\ourmethod}.
Without loss of generality, we assume that the objective function is going to be minimized.

We start from an initial reference permutation $\pi_0$ and a~\ac{PPG} with initialized weights\footnote{E.g. all the weights can be set to $0.5$} and update $\pi_0$ and the weight of the~\ac{PPG} edges using reinforcement learning.
Iteratively, we sample a permutation graph from the current~\ac{PPG} and apply the objective function to the sampled permutation $\pi$.
If $\pi$ leads to a lower objective than $\pi_0$, we replace $\pi_0$ by $\pi$ so as to have the best permutation so far as our reference permutation.
As the~\ac{PPG} is defined over the reference permutation, it should also be updated according to the new $\pi_0$.
In contrast, if $\pi$ leads to a larger value for the objective function than $\pi_0$, the edges in the sampled permutation graph will be penalized to reduce their chance of being selected in future iterations.
Our algorithm keeps the best tested permutation so far as the reference permutation and narrows down the search space each time it confronts a bad permutation, by penalizing its corresponding graph edges.

\input{sections/figure_tex/03-alg-learning}

Alg.~\ref{alg:learning} is the pseudo-code for learning the reference permutation and~\ac{PPG} weights.
It gets the initial reference permutation, $\pi_0$, as well as initial~\ac{PPG}, $G$, as input and returns the updated version of them.
It also gets the objective function to be minimized, $f$, and the learning rate, $\eta$, used for updating the weights (Line $9$).
The \textit{Not converged} condition in line $1$ can be implemented with standard stopping criteria such as a fixed number of iterations where $\pi_0$ is not updated.
In our implementation, we stop after $20$ consecutive iterations of non-changing $\pi_0$.

\todo{Update $G$ accordingly ...}




\begin{algorithm}
    \caption{{\bfseries $Sample(D,G)$} Sampling Permutation Graph}
    \label{alg:sampling}
    \SetAlgoLined
    \KwIn{$D=[d_1,d_2,\dots,d_n]$, $G=(D,E,w)$}
    \KwOut{$D'$ (a permutation on $D$, sampled from $G$)}
    Initialize $D'=D$\\% and $E_P=\emptyset$\\
    $L=[1,2,\cdots,n]$\\
    \While{$L \neq \emptyset$}{
        $L'=\emptyset$\\
        \ForAll{$i$ randomly picked from $L$}{
            $e=(D'[i],D'[i+1])$\\
            Sample $e$ with probability $w(e)$\\
            \If{$e$ is sampled}{
                Swap $D'[i]$ and $D'[i+1]$\\
                % $E_P = E_P \cup \{e\}$\\
                $L' = L' \cup \{i-1,i+1\}$\\
                $L = L - \{i-1,i+1\}$\\
            }
        }
        $L=L'$
    }
    Return $D'$
\end{algorithm}

